Im2Struct: Recovering 3D Shape Structure from a Single RGB Image

We propose to recover 3D shape structures from single RGB images, where structure refers to shape parts represented by cuboids and part relations encompassing connectivity and symmetry. Given a single 2D image with an object depicted, our goal is automatically recover a cuboid structure of the object parts as well as their mutual relations. We develop a convolutional-recursive auto-encoder comprised of structure parsing of a 2D image followed by structure recovering of a cuboid hierarchy. The encoder is achieved by a multi-scale convolutional network trained with the task of shape contour estimation, thereby learning to discern object structures in various forms and scales. The decoder fuses the features of the structure parsing network and the original image, and recursively decodes a hierarchy of cuboids. Since the decoder network is learned to recover part relations including connectivity and symmetry explicitly, the plausibility and generality of part structure recovery can be ensured. The two networks are jointly trained using the training data of contour-mask and cuboid structure pairs. Such pairs are generated by rendering stock 3D CAD models coming with part segmentation. Our method achieves unprecedentedly faithful and detailed recovery of diverse 3D part structures from single-view 2D images. We demonstrate two applications of our method including structure-guided completion of 3D volumes reconstructed from single-view images and structure-aware interactive editing of 2D images.

==> results.tex <==
% -*- compile-command: "texify --pdf --quiet decop_cvpr18.tex" -*-
% !TEX root = decop_cvpr18.tex
% (shell-command "start decop_cvpr18.pdf")


\section{Results and Evaluations}
We evaluate the two core components of our pipeline: the co-planarity network and the robust optimization. Since our network is the first trained to predict co-planarity, we evaluate it against several baselines, to justify our design choices. For the optimization, we will show both quantitative  and qualitative evaluations on scene reconstruction, especially for the cases which cannot be handled by key-point based methods.


\subsection{Training Set Explanation}
Our training data is generated from both ScanNet~\cite{} and Sun3D~\cite{} datasets. The $1516$ scenes in ScanNet are reconstructed by BundleFusion~\cite{}. $25$ scenes in Sun3D are reconstructed semi-automatically with human-assisted registration. For ScanNet, we adopt the training/testing split provided with the dataset. All $25$ Sun3D scenes and the training set ($1045$ scenes) of ScanNet are used to generate our training triplets. For evaluating our network, we also build a co-planarity benchmark using the $100$ of the testing scenes of ScanNet.
%
Each training scene contributes $10K$ triplets. About $10M$ triplets in total are generated from all training scenes, among which a half is randomly sampled and the other half is generated with the hard triplet mining heuristics.

\subsection{Co-planarity Benchmark}
We create a benchmark for evaluating co-planarity-based patch matching.
The benchmark dataset contains \num patch pairs which
are organized according to two aspects of matching hardness: patch size and pair distance.
We create three subsets with average physical patch size ranging from \num m$^2$, \num m$^2$, to \num m$^2$.
In these three subsets, the patch pairs are sampled at random distances.
For pair distance, we build another three subsets with average distance ranging from \num m, \num m, to \num m.
For each subset, the numbers of positive and negative pairs are roughly equal.
For both positive and negative, half of the data are sampled with our heuristic hard example mining.
The benchmark is provided in the supplementary material and will be made public upon acceptance.

\MATTHIAS{Add that table we have found}


\subsection{Network Evaluation}


\subsection{Registration Evaluation}
The evaluation of registration is conducted on the TUM RGB-D dataset by~\cite{sturm12iros},
for which ground-truth camera trajectories are available.
To better demonstrate the advantage of our method in handling sequences with
few frame-to-frame overlap, we generate a challenging test set, by down-sampling frames
from the TUM sequences by every $5$, $10$ and $15$, named TUM-d5, TUM-d10 and TUM-d15, respectively.

\paragraph{Quantitative Results}
To evaluate the robustness of our optimization, we first investigate
how tolerant it is to the precision rate of the co-planarity prediction.
In Figure~\ref{}, we plot the reconstruction error of our method
on the TUM dataset (original), with varying co-planarity precision.
The varying precisions are achieved by randomly disturbing the correct predictions
obtained by our network.
Reconstruction error is measured as the absolute trajectory error (ATE), i.e.,
the root-mean-square error (RMSE) of camera positions along a trajectory.
\kev{From the results, ...}

Normal estimation for planar patches is crucial to our co-planarity-based alignment.
In Figure~\ref{}, we demonstrate how our optimization is able to tolerate
noise in normals.
In reconstructing the TUM dataset, we add random noise (with a standard deviation of $5^\circ$)
to the estimated normals in each iteration, for varying percentages of patches.
\kev{The results show that our method is robust ...}


On the down-sampled TUM sequences, we compare our method
with six state-of-the-art reconstruction methods, including
RGB-D SLAM~\cite{endres2012evaluation},
VoxelHashing~\cite{niessner2013hashing},
ElasticFusion~\cite{Whelan15rss},
Redwood~\cite{choi2015robust},
BundleFusion~\cite{dai2017bundlefusion} and
Fine-to-Coarse~\cite{halber2016fine}.
Table~\ref{} reports the ATE RMSE comparison on TUM-d10. The results for TUM-d5 and TUM-d15
can be found in the supplementary material.




\begin{table}[h]\center
    \scalebox{0.9}{	
		\begin{tabular}{| c | c | c | c | c |}
			\hline
			& fr1/desk & fr2/xyz & fr3/office & fr3/nst \\ \hline
%			DVO SLAM & 2.1cm & 1.8cm & 3.5cm & 1.8cm \\ \hline
			RGB-D SLAM & 2.3cm & 0.8cm & 3.2cm & 1.7cm \\ \hline
%			MRSMap & 4.3cm & 2.0cm & 4.2cm & 201.8cm \\ \hline
%			Kintinuous & 3.7cm & 2.9cm & 3.0cm & 3.1cm \\ \hline
			VoxelHashing & 2.3cm & 2.2cm & 2.3cm & 8.7cm \\ \hline
			Elastic Fusion & 2.0cm & 1.1cm & 1.7cm & 1.6cm  \\ \hline
%			LSD-SLAM & - & 1.5cm & - & -  \\ \hline
%			Submap BA & 2.2cm & - & 3.5cm & -  \\ \hline
			Redwood (rigid) & 2.7cm & 9.1cm & 3.0cm & 192.9cm  \\ \hline
			BundleFusion  & 1.6cm & 1.1cm & 2.2cm & 1.2cm \\ \hline
            Fine-to-Coarse  & 1.6cm & 1.1cm & 2.2cm & 1.2cm \\
            \hline \hline
			Ours  & XXX & XXX & XXX & XXX \\ \hline
		\end{tabular}
		\label{tab:comp_tum}
    }
	\caption{ATE RMSE (in cm) on downsampled TUM sequences~\protect\cite{sturm12iros}, TUM-d10. Note that unlike the other methods listed, Redwood does not use color information.}
\end{table}


\paragraph{Qualitative Results}
\MATTHIAS{Here, we would pick examples that traditional key-point based methods cannot address; e.g., we where we can get loop closures of two frames where no key point overlaps to begin with}



















%\begin{table}[h]
%	\begin{center}
%		\begin{tabular}{| c | c | c | c | c |}
%			\hline
%			& kt0 & kt1 & kt2 & kt3  \\ \hline
%			DVO SLAM & 10.4cm & 2.9cm & 19.1cm & 15.2cm \\ \hline
%			RGB-D SLAM & 2.6cm & 0.8cm & 1.8cm & 43.3cm \\ \hline
%			MRSMap & 20.4cm & 22.8cm & 18.9cm & 109cm \\ \hline
%			Kintinuous & 7.2cm & 0.5cm & 1.0cm & 35.5cm \\ \hline
%			VoxelHashing & 1.4cm & 0.4cm & 1.8cm & 12.0cm \\ \hline
%			Elastic Fusion & 0.9cm & 0.9cm & 1.4cm & 10.6cm  \\ \hline
%			Redwood (rigid) & 25.6cm & 3.0cm & 3.3cm & 6.1cm  \\ \hline
%			BundleFusion  & 0.6cm & 0.4cm & 0.6cm & 1.1cm \\ \hline  \hline
%			Ours & XXX & XXX & XXX & XXX \\ \hline
%		\end{tabular}
%		\label{tab:comp_synth}
%	\end{center}
%		\caption{ATE RMSE on the synthetic ICL-NUIM dataset by~\protect\cite{handa:etal:ICRA2014}; note that unlike the other methods, Redwood does not use color information and runs offline. \MATTHIAS{I doubt we can show synthetic data without fine-tuning on it}}
%\end{table}
